52 Weeks Later: Attitudes Towards COVID-19 Apps for Different Purposes Over Time

The COVID-19 pandemic has prompted countries around the world to introduce smartphone apps to support disease control efforts. Their purposes range from digital contact tracing to quarantine enforcement to vaccination passports, and their effectiveness often depends on widespread adoption. While previous work has identified factors that promote or hinder adoption, it has typically examined data collected at a single point in time or focused exclusively on digital contact tracing apps. In this work, we conduct the first representative study that examines changes in people's attitudes towards COVID-19-related smartphone apps for five different purposes over the first 1.5 years of the pandemic. In three survey rounds conducted between Summer 2020 and Summer 2021 in the United States and Germany, with approximately 1,000 participants per round and country, we investigate people's willingness to use such apps, their perceived utility, and people's attitudes towards them in different stages of the pandemic. Our results indicate that privacy is a consistent concern for participants, even in a public health crisis, and the collection of identity-related data significantly decreases acceptance of COVID-19 apps. Trust in authorities is essential to increase confidence in government-backed apps and foster citizens' willingness to contribute to crisis management. There is a need for continuous communication with app users to emphasize the benefits of health crisis apps both for individuals and society, thus counteracting decreasing willingness to use them and perceived usefulness as the pandemic evolves.

==> acmart-preload-hook.tex <==
% For backwards references in the bibliography
% https://twitter.com/sergeyi49013776/status/1526627104032530434?s=21&t=vKg8wUcF3QthNzziFIC3gg
\usepackage[bookmarksnumbered,unicode,pagebackref=true]{hyperref}
\renewcommand*\backref[1]{\ifx#1\relax \else (cited on p. #1). \fi}

==> sections/6_limitations.tex <==
\section{Limitations}
\label{sec:limitations}
The various factors and factor levels that could occur in a COVID-19 app were created based on a set of apps from the beginning of the pandemic.
Knowing that real applications are constantly updated and that we would not be able to adjust the study design as rounds progressed, we tried to account for possible future developments.
Nevertheless, the app scenarios presented in the vignettes are theoretical and simplified and thus unlikely to accurately represent existing apps.

In our evaluations, we tried to account for changing circumstances over the course of the pandemic, such as social restrictions, newly released apps, and ongoing public discussions about COVID-19 apps.
However, due to their complexity, we cannot always assign cause and effect beyond doubt. 
Attitudes towards using a COVID-19 app might be partly influenced by political opinions. However, we did not collect data on political opinions in our questionnaire since comparing political views across countries is not trivial and was also not the focus of this work. 

Due to the study design investigating developments over time, we could not adjust the survey to reflect current developments. In particular, the factors for the CLMM model must stay the same to allow for an analysis of changes over time.
